The Forward Physics Facility at the Large Hadron Collider

The Forward Physics Facility (FPF) is a proposal developed to exploit the unique scientific potential made possible by the intense hadron beams produced in the far-forward direction at the high luminosity LHC (HL-LHC). Housed in a well-shielded cavern 627 m from the LHC interactions, the facility will enable a broad and deep scientific programme which will greatly extend the physics capability of the HL-LHC. Instrumented with a suite of four complementary detectors -- FLArE, FASER$\nu$2, FASER2 and FORMOSA -- the FPF has unique potential to shed light on neutrino physics, QCD, astroparticle physics, and to search for dark matter and other new particles. This contribution describes some of the key scientific drivers for the facility, the engineering and technical studies that have been made in preparation for it, the design of its four complementary experiments, and the status of the project's partnerships and planning.

==> header.tex <==

\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx,tabularx}
\usepackage{color}
\usepackage{multirow}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{slashed}
\usepackage[normalem]{ulem}
\usepackage{wrapfig}
\usepackage{cancel}
\usepackage{xcolor}
\usepackage{lineno}
\usepackage{datetime}


%\usepackage[nottoc]{tocbibind}
%\usepackage[letterpaper,dvips,hmargin={1in,1in},vmargin={1.2in,0.8in}]{geometry}
%\usepackage[letterpaper,dvips,hmargin={1in,1in},vmargin={1.1in,0.9in}]{geometry}
\usepackage[a4paper,margin=21mm]{geometry}

% left margin for description / itemize
%\setlist[description]{leftmargin=0.3cm}
%\setlist[itemize]{leftmargin=0.5cm}

% begin / end equation
\newcommand{\be}{\begin{equation} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\def\figureautorefname~#1\null{Fig.\,#1\null}
\def\tableautorefname~#1\null{Tab.\,#1\null}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\def\equationautorefname~#1\null{Eq.\,(#1)\null}

% cref
\crefname{section}{Sec.}{Secs.}
\crefname{chapter}{Chapter}{Chapters}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{table}{Table}{Tables}
\crefname{appendix}{Appendix}{Appendices}

% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}
\newcommand{\br}{\mathrm{BR}}

% Units
\newcommand{\ev}{\text{eV}}
\newcommand{\kev}{\text{keV}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}

\newcommand{\ab}{\text{ab}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\pb}{\text{pb}}
\newcommand{\ipb}{\text{pb}^{-1}}

\newcommand{\nm}{\text{nm}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}
\newcommand{\Dsle}[1]{\slash\hskip -0.23 cm #1}
\newcommand{\met}{{\Dsle E_T}}

\newcommand{\mrad}{\text{mrad}}
\newcommand{\murad}{\mu\text{rad}}

\newcommand{\s}{\text{s}}
\newcommand{\g}{\text{g}}
\newcommand{\kg}{\text{kg}}
\newcommand{\ton}{\text{t}}
\newcommand{\sr}{\text{sr}}
\newcommand{\ns}{\text{ns}}
\newcommand{\hz}{\text{Hz}}

\newcommand{\Eqref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\Eqsref}[2]{Equations~(\ref{eq:#1}) and (\ref{eq:#2})}
\renewcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\eqsref}[2]{Eqs.~(\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\secsref}[2]{Secs.~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Secsref}[2]{Sections~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figsref}[2]{Figs.~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\figssref}[3]{Figs.~\ref{fig:#1}, \ref{fig:#2} and \ref{fig:#3}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tableref}[1]{Table~\ref{table:#1}}
\newcommand{\tablesref}[2]{Tables~\ref{table:#1} and \ref{table:#2}}
\newcommand{\appref}[1]{Appendix~\ref{sec:#1}}
\newcommand{\appsref}[2]{Appendices~\ref{sec:#1} and \ref{sec:#2}}

%tools
\newcommand{\texttool}[1]{\texttt{#1}}

% experiment names
\newcommand{\sndfar}{\ensuremath{\text{AdvSND}_{\text{far}}}}
\newcommand{\sndnear}{\ensuremath{\text{AdvSND}_{\text{near}}}}
\newcommand{\snd}{\ensuremath{\text{SND@LHC}}}
\newcommand{\fasernu}{FASER$\nu$}

% changed comments
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}

% contributor / convener entry
\newcommand{\contributor}[1]{\noindent {\em \textbf{Contributor:} #1} \\ }
\newcommand{\contributors}[1]{\noindent {\em \textbf{Contributors:} #1} \\ }
\newcommand{\convener}[1]{\noindent {\em \textbf{Convener:} #1} \\ }
\newcommand{\conveners}[1]{\noindent {\em \textbf{Conveners:} #1} \\ }

% our comments
\newcommand{\Felix}[1]{\textcolor{magenta}{[FK: #1]}}
\newcommand{\jlf}[1]{\textcolor{red}{[JLF: {#1}]}}
\newcommand{\Seb}[1]{\textcolor{orange}{[ST: #1]}}
\newcommand{\dsol}[1]{\textcolor{cyan}{[DS: #1]}}
\newcommand{\BB}[1]{\textcolor{blue}{[BB: #1]}}
\newcommand{\tm}[1]{\textcolor{purple}{[TM: {#1}]}}
\newcommand{\fixme}[1]{\textcolor{red}{???: {#1}]}}
% depth of TOC (add first one not to be shown)
%\makeatletter
%\def\l@subsubsection#1#2{}
%\def\l@paragraph{\@dottedtocline{4}{5.3em}{2.1em}}
%\makeatother

\setcounter{tocdepth}{3}
\setcounter{secnumdepth}{3}

% introduced by Juan for QCD
%\usepackage{physics}
\usepackage{mathtools}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{pifont}

%\usepackage{todonotes}
\newcommand{\cmark}{\cellcolor{blue!20}\textcolor{blue}{\ding{51}}}%
\newcommand{\xmark}{\cellcolor{red!20}\textcolor{red}{\ding{55}}}%
\newcommand{\ymark}{\cellcolor{yellow!30}\textcolor{blue}{(\ding{51})}}%
\newcolumntype{C}{>{\centering\arraybackslash}p{1.5cm}}
\usepackage{adjustbox}

% Snowmass ``branding''
\newcommand\snowmass{
\begin{center}
  \rule[-0.2in]{\hsize}{0.01in}\\
  \rule{\hsize}{0.01in}\\
  \vskip 0.1in
  Submitted to the US Community Study\\ 
  on the Future of Particle Physics (Snowmass 2021)\\
  \rule{\hsize}{0.01in}\\
  \rule[+0.2in]{\hsize}{0.01in}\\[-2em]
\end{center}
}


% space on top/bottom from figures (copied from revtex)
\setcounter{topnumber}{2}
\def\topfraction{.9}
\setcounter{bottomnumber}{1}
\def\bottomfraction{.9}
\setcounter{totalnumber}{3}
\def\textfraction{.1}
\def\floatpagefraction{.9}
\setcounter{dbltopnumber}{2}
\def\dbltopfraction{.9}
\def\dblfloatpagefraction{.9}

%spacing in references
%\let\oldbibliography\thebibliography
%\renewcommand{\thebibliography}[1]{%
%  \oldbibliography{#1}%
%  \setlength{\itemsep}{-1pt}%
%}


% Ref Style
\bibliographystyle{utphys}
